A Random Matrix Theory Approach to Damping in Deep Learning

We conjecture that the inherent difference in generalisation between adaptive and non-adaptive gradient methods in deep learning stems from the increased estimation noise in the flattest directions of the true loss surface. We demonstrate that typical schedules used for adaptive methods (with low numerical stability or damping constants) serve to bias relative movement towards flat directions relative to sharp directions, effectively amplifying the noise-to-signal ratio and harming generalisation. We further demonstrate that the numerical damping constant used in these methods can be decomposed into a learning rate reduction and linear shrinkage of the estimated curvature matrix. We then demonstrate significant generalisation improvements by increasing the shrinkage coefficient, closing the generalisation gap entirely in both logistic regression and several deep neural network experiments. Extending this line further, we develop a novel random matrix theory based damping learner for second order optimiser inspired by linear shrinkage estimation. We experimentally demonstrate our learner to be very insensitive to the initialised value and to allow for extremely fast convergence in conjunction with continued stable training and competitive generalisation.

==> deprecated-drafts/abstract_deprecated.tex <==
\begin{abstract}
We conjecture that the reason for the difference in generalisation between adaptive and non adaptive gradient methods is the the relative lack of movement in the sharpest directions of the loss landscape. This conjecture---motivated by recent results in random matrix theory~\citep{granziol2020towards}---has implications for optimisation in both simple convex settings and deep neural networks. We show that popular modifications to adaptive methods such as decoupled weight decay \citep{loshchilov2018decoupled}, partial adaptivity~\citep{chen2018closing} and epsilon tuning~\citep{choi2019empirical} each act to increase movement along these sharp directions. By replacing conventional sharp learning rate decay schemes with iterate averaging \citep{polyak1992acceleration}, we further increase relative movement and completely close the generalisation performance gap between Adam and SGD. We provide empirical evidence of this effectiveness of our approach for the VGG and ResNet architectures on the CIFAR-$10$/$100$ and ImageNet datasets. %, Adam performs better than finely tuned SGD and by introducing partial adaptivity, Adams performance is even better than SGD with iterate averaging, whilst still converging faster.
Finally, we compare our algorithms with the recently proposed Lookahead optimiser \citep{zhang2019lookahead} and show some complementary benefit of the two approaches.
We posit that previous attempts to combine adaptive gradient methods with iterate averaging failed to materialise in improved generalisation due to the lack of movement in sharp directions, which the aforementioned techniques rectify. 

% We conjecture that the reason for the difference in generalisation between adaptive and non adaptive gradient methods is the the relative lack of movement in the sharpest directions of the loss landscape. This conjecture is motivated by random matrix theory~\citep{granziol2020towards} and stability analysis~\citep{wu2018sgd}. We demonstrate that this impacts generalisation in both a convex setting and a deep neural network. We show that heuristics shown to improve the generalisation of adaptive methods, such as decoupled weight decay \citep{loshchilov2018decoupled}, partial adaptivity \citet{chen2018closing} and epsilon tuning \citet{choi2019empirical} can be seen as special cases of increasing movement along these directions. By replacing conventional sharp learning rate decay schemes with iterate averaging \cite{polyak1992acceleration}, further increasing the relative movement in these sharp directions, we completely close the generalisation performance gap between Adam and SGD. We find that by including this small modification, for the VGG and ResNet architectures on the CIFAR-$10$/$100$ and ImageNet datasets, Adam performs better than finely tuned SGD and by introducing partial adaptivity, Adams performance is even better than SGD with iterate averaging, whilst still converging faster. We compare our algorithms against the recently proposed Lookahead optimiser \citep{zhang2019lookahead} and show some combinable benefit of the two approaches.
% We posit that previous attempts to combine adaptive gradient methods with iterate averaging failed to materialise in improved generalisation due to the lack of movement in these sharp directions, which the aforementioned techniques rectify. 

%We posit that previous attempts to combine adaptive gradient methods with Polyak averaging failed to materialise in improved generalisation due to the lack of movement in these sharp directions, which the aforementioned techniques rectify. 
%
%This insight informs a practical algorithm, where we simply combine these aforementioned techniques with iterate averaging \cite{polyak1992acceleration} instead of traditional sharply decaying learning rates. This allows for a higher effective learning rate in the sharpest directions throughout training. We posit that previous attempts to combine adaptive gradient methods with Polyak averaging failed to materialise in improved generalisation due to the lack of movement in these sharp directions, which the aforementioned techniques rectify. 
%We show that even without compromising adaptivity and at minimal additional computational burden, that our algorithm achieves a generalisation performance that is consistently superior to tuned SGD and is even on par or better compared to SGD with iterate averaging on various image classification (CIFAR 10/100 and ImageNet) and language tasks (Penn Tree Bank). 
	
%Iterate averaging has a rich history in optimisation, but has only very recently been popularised in deep learning. We investigate its effects in a deep learning context, and argue that previous explanations on its efficacy, which place a high importance on the local geometry (flatness vs sharpness) of final solutions, are not necessarily relevant. We instead argue that the robustness of iterate averaging towards the typically very high estimation noise in deep learning and the various regularisation effects averaging exert, are the key reasons for the performance gain, indeed this effect is made even more prominent due to the over-parametrisation of modern networks. Inspired by this, we propose Gadam, which combines Adam with iterate averaging to address one of key problems of adaptive optimisers that they often generalise worse. Without compromising adaptivity and with minimal additional computational burden, we show that Gadam (and its variant GadamX) achieve a generalisation performance that is consistently superior to tuned SGD and is even on par or better compared to SGD with iterate averaging on various image classification (CIFAR 10/100 and ImageNet 32$\times$32) and language tasks (PTB).
\end{abstract}

==> deprecated-drafts/conjecture_deprecated_v1.tex <==
\section{Direction as well as step size determines generalisation} \label{sec:motivation}

\begin{figure}[h!]
	\centering
	\begin{subfigure}[b]{0.45\textwidth}
		\includegraphics[width=\textwidth]{figs/IClR_simple_Adam_simple}
		\vspace{-15pt}
		\caption{Adam various learning rates}
		\label{subfig:adaptivegaplr}
	\end{subfigure}
	\begin{subfigure}[b]{0.49\textwidth}
		\includegraphics[width=\textwidth]{figs/IClR_adamvssgd_Adam}
		\vspace{-15pt}
		\caption{SGD and Adam largest learning rate}
		\label{subfig:sgdvsadam}
	\end{subfigure}
	%	\begin{subfigure}
	\vspace{0pt}
	\caption{Training and Validation error for Adam/SGD on the VGG-$16$ \& CIFAR-$100$ dataset with no weight decay or batch norm for various learning rates, batch size $B=128$}
	\label{fig:lrimportance}
	\vspace{-10pt}	
\end{figure}
The learning rate to batch size ratio has been shown to correlate with generalisation for SGD \citet{jastrzkebski2017three} and under the dynamical stability perspective of SGD \citet{wu2018sgd}, utilising larger learning rates select flatter minima, which under a Bayesian and minimum description length framework \citet{hochreiter1997flat}, generalise better. For Adam similarly, as shown in Figure \ref{subfig:adaptivegaplr}, larger learning rates lead to better generalisation, despite lower learning rates quickly training better. For this experiment we use the classical VGG-$16$ network \citep{simonyan2014very} and we compare $\alpha = 0.0004$ which is the largest learning rate of stable training\footnote{We test this for multiple seeds.}, to a smaller learning rate. As shown in Figure \ref{subfig:sgdvsadam},
even when using the respective maximal learning rates for SGD $\alpha=0.01$ and Adam, SGD still generalises better. This is without batch normalisation \citet{ioffe2015batch} or the use of weight decay, so is not addressed in the work of \citet{loshchilov2018decoupled}. Furthermore, even though the global maximal learning rate of Adam is smaller than that of SGD, $\alpha_{Adam} = 0.0004 \ll \alpha_{SGD} = 0.01$, Adam scales its parameter updates by an inverse square root weighted average of gradient squares plus a small offset $\epsilon = 10^{-8}$ for numerical stability. Hence, the largest per parameter learning rate possible is $4\times 10^{4} \gg \alpha_{SGD}$. This shows that whilst effective for SGD, the global learning rate is too crude to analyse the behaviour of adaptive algorithms and a more detailed analysis is required.

\paragraph{Second Order Optimisers:}solve the quadratic as opposed to the linear approximation around the loss $L(\vw_{k})$ at point $\vw_{k}$. Writing the update in the eigenbasis of the Hessian $\mH = \nabla^{2}L(\vw_{k}) = \sum_{i}^{P}\lambda_{i}\vphi_{i}\vphi_{i}^{T} \in \mathbb{R}^{P\times P}$ the updated step is given as:
\begin{equation}
\label{eq:secondorderopt}
\vw_{k+1} = \vw_{k} - \alpha \mH^{-1}\nabla L(\vw_{k}) = \vw_{k} - \sum_{i=1}^{P}\frac{\alpha}{\lambda_{i}+\delta}\vphi_{i}\vphi_{i}^{T}\nabla L(\vw_{k})
\end{equation}
Where $\vw_{k}$ are the model weights at iteration $k$, $[\vphi_{i},\lambda_{i}]$ are the eigenvalues/eigenvector pairs of $\mH$, $\alpha$ is the global learning rate and $\delta$ is a damping term, often grid searched \citet{dauphin2014identifying} or adapted during training \citet{martens2015optimizing}. It can be considered a trust region and is required to stop the optimiser moving too far in directions deemed flat ($\lambda_{i} \approx 0$) and diverging. The exact computation of $\mH^{-1}$ is extremely expensive when $P$ is large (as full eigen-decomposition has computational complexity $\mathcal{O}(P^{3})$). Hessian vector products \citep{pearlmutter1994fast} have been used to approximate the Hessian \citep{martens2010deep,dauphin2014identifying}, along with KFAC, which uses a Kronecker factored approximations of the Fisher information matrix \citep{martens2015optimizing}.

As can be seen from Equation \ref{eq:secondorderopt}, the effective learning rate in the flattest directions is given by $\frac{\alpha}{\delta}$, which is larger than that in the sharpest direction $\frac{\alpha}{\delta+\lambda_{1}}$. From a dynamical stability perspective \citet{wu2018sgd}, reducing the effective learning rate in the sharp directions means the optimiser is likely to get stuck into a sharp optimum, which generalises worse. The key result adapted from the spiked covariance literature to deep learning \citet{granziol2020curvature}, holding under quite general conditions (given in the Appendix), which we state:
\begin{theorem}
	\label{theorem:overlap}
	The eigenvector overlap between the eigenvectors $\hat{\vphi}_{i} \in \mathbb{R}^{P 
		\times 1}$ of the Hessian of the mini-batch $\nabla^{2}L_{batch}(\vw_{k})$ of batch size $B$ and the eigenvectors $\vphi_{i}$ of the Hessian under the expectation of the true data distribution $\nabla^{2}L_{true}(\vw_{k})$, where $L_{true}(\vw_{k}) = \int \ell(\vw_{k};\vx,\vy)d\phi_{\vx,\vy}$ are given by
	\begin{equation}
	|\hat{\vphi}_{i}^{T}\vphi_{i}|^{2} = \begin{cases} 1-\frac{P\sigma^{2}}{B\lambda_{i}^{2}} &\mbox{if } |\lambda_{i}| > \sqrt{\frac{P}{B}}\sigma\\
	0 & \mbox{otherwise} \end{cases}  
	\end{equation}
\end{theorem}
Where $\sigma$ captures the sampling noise, present even for the full gradient $B=N$. Hence the sharp directions represent the signal in our gradient and Equation \ref{eq:secondorderopt} is reduces our signal to noise ratio in our parameter updates. %This is known as the eigenvector phase transition \citep{baik2005phase}. The gradient is a function of curvature\footnote{using a local quadratic expansion $\nabla L = \sum_{i}^{P}\vphi_{i}^{T}\vw(1-\alpha\lambda_{i})\vphi_{i}$} and hence the directions of the true and sampled loss vary is pertinent to generalisation difference. By Theorem \ref{theorem:overlap}, as only the sharpest directions retain information about the true loss, the last thing we want to do is move less in these directions. This is exactly what second order and adaptive gradient methods do, as shown in Equation \ref{eq:adamvssgd}.
\subsection{Experimental Validation: LanczosOPT on Logistic Regression MNIST}
\label{subsec:logisticexp}
We validate our conjecture that movements in the sharp direction of the loss landscape are vital to generalisation, as opposed to just stability arguments, we run a convex non stochastic example. We implement a Lanczos second order (LanczosOPT) \citet{meurant2006lanczos} and gradient descent optimiser on a sub-set of $1000$ MNIST \citet{lecun1998mnist} training examples with Logistic Regression and validate on a held out test set of $10,000$. The number of outliers well seperated from the bulk of the spectrum is at most the number of classes \citet{papyan2018full} (which is $n_{c}=10$ for this dataset) and we expect that Lanczos algorithm to pick out these well seperated outliers when the number of iterations $k \gg n_{c}$ \citet{granziol2019mlrg,meurant2006lanczos}. Hence we use $k=50$.
In order to not limit ourselves to the Krylov subspace given by the sharpest directions, we specifically add back in the other directions, as shown in Equation \ref{eq:lanczosopt} where $P=7850$.
\begin{equation}
\label{eq:lanczosopt}
\vw_{k+1} = \vw_{k} -\alpha\bigg(\sum_{i}^{k}\frac{1}{\lambda_{i}+\delta}\vphi_{i}\vphi_{i}^{T}\nabla L(\vw_{k})+\sum_{k+1}^{P}\frac{1}{\delta}\vphi_{i}\vphi_{i}^{T}\nabla L(\vw_{k})\bigg)
\end{equation}
Hence for a fixed $\alpha$, by reducing/increasing $\delta$ we can increase/reduce the extent to which the flat directions dominate the sharpest directions in terms of effective learning rate\footnote{as for sharp directions $\lambda \gg \delta$}. As can be seen from Figure \ref{fig:logisticlrandeps}, for the same learning rate of $\alpha=0.01$. Reducing the damping $\delta$ quickly improves the training convergence but translates to worse generalisation. All LanczosOPT runs generalise worse than SGD. However for very large damping $\delta=1$, which posts the slowest convergence (even slower than SGD) the difference is minimal.czos
\begin{figure}[h!]
	\centering
	\vspace{-5pt}
	\begin{subfigure}[b]{0.55\textwidth}
		\includegraphics[width=\textwidth]{figs/Logistic_Gen_train}
		\caption{Training Error}
	\end{subfigure}
	\begin{subfigure}[b]{0.39\textwidth}
		\includegraphics[width=\textwidth]{figs/Logistic_Gen_test}
		\caption{Test Error}
	\end{subfigure}
	%	\begin{subfigure}
	\caption{Error for LanczosOPT/GD optimisers on Logistic Regression \& the MNIST dataset with learning rate $\alpha=0.01$ and damping $\delta$}
	\label{fig:logisticlrandeps}
	\vspace{-15pt}	
\end{figure}

In the Lanczos** run indicated by the dotted red line on the plot, we scale the eigenvalues in the denominator of Equation \ref{eq:lanczosopt} by a factor of $1000$. Whilst the maximal training through the trajectory only drops by $0.6\%$, the generalisation drops by $2.28\%$. 

\subsection{Experimental Validation: KFAC VGG-16 CIFAR100:}
%For the same experimental setup as in Section \ref{sec:motivation}, we plot the training and validation error of the second order optimiser KFAC in Figure \ref{fig:kfaclrandeps}.
To show that our conjecture has practical consequences for modern deep learning architectures, we run the second order optimiser KFAC \citep{martens2015optimizing} on the VGG-$16$ for the CIFAR-$100$ dataset.  We lower the global learning rate, keeping $\alpha/\delta$ constant so our effective learning rate $(\frac{\lambda}{\alpha} + \frac{\delta}{\alpha})^{-1}$ is principally lowered in the sharp directions. As shown in Figure \ref{fig:kfaclrandeps} the training performance improves slightly $99.85\% \rightarrow 99.92 \%$, but the generalisation performance decreases $65\%\rightarrow62.2\%$. The largest learning rate posts a similar generalisation performance to that of SGD $65.3\%$. For large learning rates, decreasing the damping results in poor training, shown as dotted lines in the Figure. However for very low learning rates typically used in practice for both adaptive and second order regimes, the network efficiently trains with a lower damping co-efficient as $\lambda_{min}/\alpha \gg \delta/\alpha$. Whilst these regimes train similarly well, they generalise more poorly. For $\alpha = 0.0001$ dropping the damping co-efficient $\epsilon$ from to $0.0003$ and $0.0001$ drops the generalisation further to $60.2\%$ and then $56\%$ respectively. For both cases, the drop in generalisation is significantly larger than the drop in training accuracy. We investigate whether the solution generalisation is related to the sharpness of the end point by running the Lanczos algorithm on the entire dataset at the end of training and show the results in Figure \ref{fig:tableofspectralnormkfac}. We find that for this experiment that lower learning rates whilst keeping $\alpha/\delta$ constant increase the spectral norm and decreases generalisation. Also that decreasing $\delta$ whilst keeping $\alpha$ constant, further increases the spectral norm and decreases generalisation. This shows that damping as well as the learning rate is important for flatness and generalisation.
\begin{figure}[h!]
	\vspace{-20pt}
	\begin{minipage}{0.70\textwidth}
		\begin{subfigure}[b]{0.66\textwidth}
			\includegraphics[width=\textwidth]{figs/gen_train_kfac_VGG16_CIFAR100}
			%		\caption{VGG-16}
		\end{subfigure}
		\hspace{-15pt}
		\begin{subfigure}[b]{0.37\textwidth}
			\includegraphics[width=\textwidth]{figs/gen_test_kfac_VGG16_CIFAR100}
			%		\caption{PRN-110}
		\end{subfigure}
		%	\begin{subfigure}
		\vspace{-20pt}
		\caption{Training/Validation error for KFAC on the VGG-$16$ \& CIFAR-$100$ dataset using various learning rates $\alpha$ and damping $\delta$}
		\label{fig:kfaclrandeps}
		\vspace{-20pt}
	\end{minipage}	
	\begin{minipage}{0.29\textwidth}
		\vspace{25pt}
		\begin{scriptsize}
			\begin{tabular}{@{}llll@{}}
				\toprule
				$\delta \downarrow, \alpha \rightarrow$& 0.01 & 0.001 & 0.0001 \\ \midrule
				0.1 &  \textbf{6.65} & \textbf{} & \textbf{} \\
				0.01 & \textbf{} &  \textbf{20.8} & \textbf{} \\
				0.001 & \textbf{} & \textbf{} & \textbf{48.2} \\
				0.0003 & \textbf{} & \textbf{} &  \textbf{527.2} \\
				0.0001 & \textbf{} & \textbf{} &  \textbf{711.3} \\ \bottomrule
			\end{tabular}
		\end{scriptsize}
		\vspace{6pt}
		\caption{$|\mH|$ at training end for various $\alpha,\delta$}
		\label{fig:tableofspectralnormkfac}
		\vspace{0pt}
	\end{minipage}
\vspace{-5pt}
\end{figure}

%\begin{conjecture}
%	\label{conjecture:main}
%	The step size in the sharpest directions of the loss landscape (as defined by the eigenvectors corresponding to the largest eigenvalues of the Hessian of the loss) is a key explanatory factor of the generalisation performance.
%\end{conjecture}

%We believe that both the generalisation gap between different networks trained with learning rates and the adaptive generalisation gap, can be explained with the following conjecture, which forms the


%To isolate the learning rate from the interfering effects of batch normalisation (BN) \citep{ioffe2015batch} and weight decay (wd) (decoupled or not), we use the classical VGG-$16$ network \citep{simonyan2014very} without batch normalisation and no weight decay on the CIFAR-$100$ dataset classification task. As shown in Figure \ref{subfig:adaptivegaplr}, for Adam similarly to SGD \citep{jastrzkebski2017three}, a large learning rate to batch size ratio leads to greater generalisation. We compare $\alpha = 0.0004$ which is the largest learning rate of stable training\footnote{We test this for multiple seeds.}, to a smaller learning rate.
%We note here that the lower learning rate regime quickly trains better, but generalises worse. Even when using the respective maximal learning rates for SGD and Adam, as shown in Figure \ref{subfig:sgdvsadam}, SGD still generalises better.We believe that both the generalisation gap between different networks trained with learning rates and the adaptive generalisation gap, can be explained with the following conjecture, which forms the focal point of our analysis
%\begin{figure}[h!]
%	\vspace{-10pt}
%	\centering
%	\includegraphics*[width=0.9\textwidth]{figs/IClR_simple_Adam_simple}
%	\vspace{-10pt}
%	\caption{Adam training and validation error curves on the VGG-$16$ network and CIFAR-$100$ dataset, for different learning rates $\alpha$ but fixed batch size $B=128$}
%	\label{fig:adaptivegaplr}
%	\vspace{-10pt}
%\end{figure} 
%which shows the training and test error of the VGG-$16$ without weight decay nor batch normalisation (BN) \citep{ioffe2015batch} for the CIFAR-$100$ dataset under different learning rates. $\alpha = 0.0004$ is the maximal learning rate for which Adam stably trains\footnote{We test this for multiple seeds.} and we compare to another lower learning rate $\alpha = 0.0001$. The experimental details are given in \ref{sec:experimentdetails}. 
%Whilst the mechanisms of how large learning rates aid generalisation are not fully understood, \citet{li2019towards} show that the learning rate size affects the order in which patterns are learned. Specifically that small learning rates are able to memorise small parts of the image which may be spurious \footnote{A well known example of this is the idea that not all sports cars are red, but they often feature in training sets}. 

%\begin{figure}[h!]
%	\vspace{-10pt}
%	\centering
%	\includegraphics*[width=0.9\textwidth]{figs/IClR_adamvssgd_Adam}
%	\vspace{-10pt}
%	\caption{SGD and Adam training/validation error curves on the VGG-$16$ network and CIFAR-$100$ dataset, for different learning rates $\alpha$ but fixed batch size $B=128$}
%	\label{fig:adaptivegap}
%	\vspace{-10pt}
%\end{figure}


\section{Explicit Link to Adaptive Gradient Methods}
%\paragraph{Optimisation and Generalisation:}For a data-set of $N$ training input-output samples $\{\vx_i, \vy_i\}$ and a model parametrised by $\vw \in \mathbb{R}^P$, for a given loss function $\ell(h(\vx_{i};\vw),\vy_{i})$ the \emph{empirical risk} also known as the training loss in deep learning is given by $R_{emp}(\vw) = \frac{1}{N}\sum_{i=1}^{N}\ell(h(\vx_{i};\vw),\vy_{i})$. For a randomly sampled mini-batch of size $B$ from the training set, the batch risk is given $R_{batch}(\vw) = \frac{1}{B}\sum_{i=1}^{N}\ell(h(\vx_{i};\vw),\vy_{i})$, which is considered as an estimate of the empirical risk and used in deep learning optimisation. Ideally we would optimise the \emph{true risk}, $R_{true}(\vw) = \int \ell(h(\vx;\vw),\vy_{i})d\phi_{\vx,\vy}$ under the data-generating distribution $\phi_{\vx,\vy}$. The loss using a held out test set can be seen as an unbiased estimate of the true risk.  Given the inherent unobservability of true risk, the minimisation or $R_{emp}$ is considered to be the practical optimisation problem of network training \cite{bottou2018optimization}. The generalisation gap is given by $R_{true}(\vw) - R_{emp}(\vw)$ and can be estimated by reporting the difference between the training and test loss. The adaptive generalisation gap is the difference between the generalisation gaps between adaptive and non adaptive optimisers. Whilst the cross entropy loss $l(h(\vx_{i};\vw),\vy_{i})$ is used in the optimisation procedure, keeping in line with existing literature we will report the frequency of misclassification as a measure of risk. Since for modern DNN's training error is usually very low, we simply report the misclassification on the test set as our measure of generalisation. The nabla $\nabla$ and del $\nabla^{2}$ operators define the gradients and Hessians on the empirical, true and batch risks respectively.
Ignoring additional features such as momentum and explicit regularisations, the $k+1$-th iteration of a general iterative optimiser is given by:
\begin{equation}
\vw_{k+1} \leftarrow \vw_{k} - \alpha \mB^{-1} \nabla L(\vw_{k})
\end{equation}
For SGD, the preconditioning matrix $\mB = I$ whereas for adaptive methods, $\mB$ typically approximates the Hessian $\mB \approx \nabla^{2}L(\vw_{k})$ information. Adaptive gradient methods use past gradient information to create a diagonal approximation to the Hessian. For example, Adam uses the square root of the moving uncentered second moment of the per-parameter gradient \cite{kingma2014adam}. Adams update rule can be seen as a running diagonal approximation to the covariance of gradients, which has been shown to be closely related to the Hessian \citep{zhang2019algorithmic,jastrzebski2020the}.
%The exact computation is extremely expensive when $P$ is large (as full eigen-decomposition has computational complexity $\mathcal{O}(P^{3})$). Hessian vector products \citep{pearlmutter1994fast} have been used to approximate the Hessian \citep{martens2010deep,dauphin2014identifying}, along with KFAC, which uses a Kronecker factored approximations of the Fisher information matrix \citep{martens2015optimizing}. However, more commonly used adaptive gradient methods use past gradient information to create a diagonal approximation to the Hessian. For example, Adam uses the moving uncentered second moment of the per-parameter gradient \cite{kingma2014adam}. 
\paragraph{A closer look at the Adam and SGD updates:}
Let us consider the update equations for both SGD and Adaptive gradient methods in the basis of the eigenvectors of the Hessian. We assume that the pre-conditioning matrix $\mB \approx \mH$. We also assume that $L2$ regularisation of magnitude $\gamma$ is employed. The $\vw_{k+1}$'th weight vector is given by:
\begin{equation}
\label{eq:adamvssgd}
\vw_{k+1} = \begin{cases} {\color{blue}{(1-\gamma\alpha)\sum_{i}^{P}\vphi_{i}\vphi_{i}^{T}\vw_{k}}} - {\color{red}{\alpha\sum_{i}^{P}\vphi_{i}^{T}\nabla L(\vw)\vphi_{i}}}\ &\mbox{if SGD} \\
{\color{blue}{\sum_{i}^{P}(1-\frac{\gamma\alpha}{\lambda_{i}+\delta})\vphi_{i}\vphi_{i}^{T}\vw_{k}}} - {\color{red}{\alpha\sum_{i}^{P}\frac{\vphi_{i}^{T}\nabla L(\vw)}{\lambda_{i}+\delta}\vphi_{i}}}  & \mbox{if Adam} \end{cases}
\end{equation}
Where for simplicity we omit momentum related terms and the damping $\delta$ is set to $10^{-8}$ in Adam.
%. and often grid searched in second order optimisers \citep{dauphin2014identifying}. \citet{chen2018closing} propose the idea that the real generalisation culprit is the small learning rate which typically accompanies adaptive methods.  For flat directions $\lambda \approx 0$, the effective learning rate is $\approx \alpha/\epsilon$, typically much larger for Adam $\approx 10^{4}$ than for for SGD $\approx 10^{-2}$. Since $\alpha$ must be chosen such that $\alpha/\epsilon$ is not too large to prevent divergence, what is much smaller is the effective learning rate for sharp directions of the loss landscape, i.e the directions where $\lambda \gg \epsilon$. Furthermore, as can be seen from Equation \ref{eq:adamvssgd}, effective weight decay in these directions is also very small. 
\paragraph{Explaining previous work under this framework:} \emph{Decoupled weight decay} \citet{loshchilov2018decoupled} simply alters Adam such that the weight decay update (shown in blue) resembles that of SGD instead of that of Adam. This effectively increases the weight decay along the sharpest directions of the loss. This increases the effective learning rate in these directions. To demonstrate this, we consider the difference in channel weight vector direction $\hat{\vw_{k}}$ \citep{hoffer2018norm} in the basis of the sharpest eigenvectors after one update of SGD
\begin{equation}
\label{eq:bndirect}
\sum_{i}^{P}\vphi_{i}\vphi_{i}^{T}\bigg(\hat{\vw}_{k+1}-\hat{\vw}_{k}\bigg) = \frac{-\eta}{||\vw_{k}||^{2}}\bigg(\mI-{\color{purple}{\sum_{i}^{P}\vphi_{i}\hat{\vw_{k}}^{T}\nabla L(\hat{\vw}_{k})\vphi_{i}^{T}\hat{\vw}_{k}}}\bigg)
\end{equation}
Hence decoupled weight decay, which by the blue term in Equation \ref{eq:adamvssgd} reduces the component along $\vphi_{i}^{T}\hat{\vw_{k}}$, through the reduction of the corrective term on the RHS of \ref{eq:bndirect} shown in purple, increases the effective learning rate. 
In Padam \citet{chen2018closing} by changing the square root in the Adam update to an arbitrary power $p < 1/2$, increases both the weight decay and the update in the sharp directions (shown in red in Equation \ref{eq:adamvssgd}), increasing the effective learning rate. Epsilon tuning \citet{choi2019empirical}, by increasing both $\epsilon$ and $\alpha$ increases both the weight decay (blue) and update in the direction of the sharpest eigenvectors (red).


%Although we do not explicitly calculate curvature information using gradient based methods, the gradient is closely aligned with
\section{Iterate Averaging: the generalisation magic bullet}

Iterate averaging (IA) \cite{polyak1992acceleration} performs a simple average of the iterates in the weight space\footnote{an average of the model parameters during training} i.e $\vw_{IA} = 1/n \sum_{i}^{n}\vw_{i}$, where $n$ is the iteration number. IA, along with learning rate reduction, is a key component for traditional convergence proofs \citep{duchi2018introductory}. 
%For the convergence proofs of all gradient based methods the average regret which is bounded can be seen as an upper bound on the loss of the iterate average \cite{duchi2018introductory,duchi2011adaptive,reddi2019convergence} (we elaborate this in App. \ref{sec:optimisationaveraging}). 
IA is optimal for stochastic problems with learning rate decay less than $1/n$, extensively observed in practice \citep{kushner2003stochastic}. As shown in Appendix \ref{subsec:noisyquad}, its noise reduction properties are superior to that exponentially moving averages which is considered to work better in practice \citep{martens2014new,zhang2019lookahead}.
%Despite these strong theoretical results, it has often been labelled as a theoretical tool that is not practically useful possibly due to the worse convergence \cite{trivedi2017}. \citet{defazio2019ineffectiveness} found that when combined with traditional learning rate scheduling IA gave poorer test performance than using the final iterate. 
Recent works have shown that averaging only at the end of training (known as \emph{tail averaging}) whilst maintaining a high learning rate, that generalisation can be significantly improved over that of traditional schedules  \cite{izmailov2018averaging,maddox2019simple, merity2017regularizing}. 
The computationally cheaper alternative of averaging every epoch instead of iteration is denoted as \textit{SWA} \citet{izmailov2018averaging}. We compare the importance of averaging frequency in Section Appendix \ref{sec:avgfreq}. Despite being mentioned as a potential modification in the original Adam paper and recommended for transformers \cite{popel2018training}, it is not typically used for image problems. Given that SGD + IA has been shown achieve large scale generalisation performance gains for both image and language problems \citet{merity2017regularizing}, along with the fact that IA is well known, this begs the question, \textit{Why doesn't iterate averaging work well for adaptive optimisers?} and more importantly \textit{can it be made to work well for adaptive optimisers?}

\paragraph{Gadam: Adapting Adam so it works well with Iterate Averaging.}
\label{sec:regularise}
Naively combining Adam with IA (AdamIA) does not lead to the same generalisation benefit as SGD with IA (SGD/SWA), as shown in Figure \ref{fig:adamvsadamw}. Model ensembling requires a diverse set of models, i.e a large learning rate. However from Equation \ref{eq:adamvssgd}, movement along the sharpest directions of the loss is much smaller for Adam than for SGD. Hence in these crucial directions, the models are not diverse. One simple remedy for this is to combine IA with decoupled weight decay. As discussed in the previous section, for modern CNNs universally equipped with BN, using decoupled weight decay increases the effective learning rate in these directions. we term this amendment to Adam, combining iterate averaging at the tail, decoupled weight decay and large learning rate \textit{Gadam}, which stands for Generalising-Adam to emphasise our focus on test not training performance. We hence expect Gadam to perform better on BN networks.
%Not only does this increase the regularisation effect along these directions, but as modern CNNs are almost universally equipped with normalisation schemes such as BN, weight reduction further acts to maintain an effective learning rate $\alpha_{\mathrm{eff}} \propto \frac{\alpha}{||\vw||^2}$ \cite{zhang2018three}. 
\begin{figure}[h!]
	\vspace{-2mm}
	\centering
	\begin{minipage}{0.6\textwidth}
		\begin{subfigure}[b]{0.49\textwidth}
			\includegraphics[width=\textwidth]{figs/bnvsnobn.png}
			\caption{Validation Accuracy}
		\end{subfigure}
		\begin{subfigure}[b]{0.46\textwidth}
			\includegraphics[width=\textwidth]{figs/ratio.png}
			\caption{Effective LR ${\alpha}/{||\vw||^2}$}
		\end{subfigure}
		\caption{Val. accuracy and $\frac{\alpha}{||\vw||^2}$ of CIFAR-100 \newline on the VGG-$16$ with/without BN. In (b) only results \newline with BN where the quantity is relevant are shown.}
		\label{fig:regularisation}    
	\end{minipage}\hfill
	\begin{minipage}{0.38\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figs/adamlinfnorm.png}  % second figure itself
		\caption{Comparing IA using Adam and AdamW on PRN-110 on CIFAR-100.}
		\label{fig:adamvsadamw}
	\end{minipage}
	\vspace{-10pt}
\end{figure}

To validate our intuition, we run a classical VGG-$16$ network on CIFAR-$100$ with and without BN (Fig. \ref{fig:regularisation}(a)): under the identical set-up, the margin of improvement of Gadam is much larger with BN. While Gadam keeps $\frac{\alpha}{||\vw||^2}$ high, in scheduled AdamW it quickly vanishes once we start learning rate decay, as shown in Figure \ref{fig:regularisation}(b). We consider whether using AdamW without schedules or with more moderate schedules can counteract this effect. However, both alternatives underperform the scheduled AdamW by more than $5\%$ (results not shown in the graph). Revisiting Figure \ref{fig:adamvsadamw} Gadam achieves a generalisation performance on par with SWA while converging faster. The more effective regularisation of AdamW is more directly shown by the much more modest weight norm growth compared to Adam during training (red lines).

%We believe the same regularisation argument also explains why combining adaptive methods with IA has \textit{not} been popularised despite the popularity of the former and the theoretical desiderata of the latter. Indeed we find naively combining Adam with IA is ineffective on typical image problems, but we argue that the real culprit is the ineffective yet commonly used $L_2$ regularisation, which counter-intuitively penalises parameters with more fluctuating gradients \textit{less} than otherwise \cite{loshchilov2018decoupled}, reducing the regularising effect and generalisation benefits IA provides. On the other hand, by penalising parameters equally, AdamW \cite{loshchilov2018decoupled} is a more effective regulariser moderating weight norm increase and we expect IA to be more effective. 

%We validate it Fig. \ref{fig:adamvsadamw}: even though Adam (blue solid lines) performs better than SGD (blue dotted lines) before $T_{\mathrm{avg}}$, the gain from averaging in final accuracy is much less. 




%
%We further argue that IA improves generalisation in networks by maintaining a high \emph{effective} learning rate, which is shown to be a strong regulariser that leads to improved generalisation of Adam and SGD \cite{zhang2018three}. This is obviously made possible by the high (nominal) learning rate schedules of IA, but on networks with batch normalisation (BN), \emph{weight reduction} is also relevant. This can be straightforwardly shown by the Cauchy-Schwartz inequality:
%\begin{theorem}
%	\label{theorem:1}
%	If iterates $\{\vw_i\}$ are drawn from a uniform distribution in the weight space, then the $L_2$ norm of the expected IA point is smaller or equal to the expectation of the $L_2$ weight norm of the iterates: $||\mathbb{E}(\vw_i)||_2^2 \leq \mathbb{E}\big(||\vw_i||_2^2\big)$ (Proof in App. \ref{sec:derivations})
%\end{theorem}
%




 %Given the widespread adoption of adaptive methods, their fast convergence along with the theoretical and practical value of iterate averaging demonstrated on SGD, this question needs further attention and is the subject of this paper.

%Originally optimisation and is actually required in all convergence proofs (we elaborate this in App. \ref{sec:optimisationaveraging}),


%In this work, instead of trading off adaptivity, we propose incorporating  \emph{iterate averaging} (IA) in Adam, an approach we term \textbf{Gadam}, to achieve the same objective. 
%While IA has a strong theoretical foundation in optimisation, it has not been often used in practice until recently:  previous works \cite{izmailov2018averaging, maddox2019simple} have applied IA with first-order optimisers (termed SWA), but to our knowledge the combination of IA and adaptive optimisers has not been thoroughly explored apart from a closely related work \cite{zhang2019lookahead}, which we compare empirically in our paper. Both drawing from prior work and developing new insights in modern deep learning, we first explore theoretically on the mechanisms of action of Gadam and critically examine the oft-held beliefs of IA.  We then empirically show that our algorithm consistently outperforms test performances of finely-tuned SGD and is competitive against SGD with iterate averaging, without compromising adaptivity or introducing sensitive new hyper parameters, in image classification (CIFAR 10/100, ImageNet 32$\times$32) and natural language processing (Penn Treebank, PTB). Finally, we demonstrate the versatility of our approach: we show that by combining Gadam with partial adaptivity (which we term \textbf{GadamX}), empirical results can be further improved, to even outperform SGD with iterate averaging yet still converge faster.

%\subsection{Iterate Averaging}

==> deprecated-drafts/conjecture_deprecated_v2.tex <==
\section{The role of relative step sizes in sharp and flat directions} \label{sec:motivation}

In Sec.~\ref{subsec:framework} below, we first describe the theory that motivates our generalization conjecture and how it relates to adaptive optimisers.
%---namely that the difference in step sizes taken along the sharpest and flattest directions of the loss landscape play a critical role in determining the generalization of adaptive methods.
We provide empirical evidence to support our claims in Sec.~\ref{subsec:logisticexp} and relate our conjecture to prior techniques in Sec.~\ref{subsec:prior-comp}. Finally, we show how \textit{iterate averaging} fits into this framework and introduce the proposed Gadam optimiser in Sec.~\ref{subsec:ia}.

\subsection{Theory: sharper directions are estimated more accurately}
\label{subsec:framework}
% \samuel{TODO: Introduce the notation i.e. say that $\vw_{k} \in \mathbb{R}^P$ represents model parameters and state that our objective is to minimise a scalar loss $L$ etc.}
% \diego{Sam: I would argue that the one should introduce the true, empirical and batch loss kind of page $3$ \hyperlink{https://arxiv.org/pdf/2006.09092.pdf}{here}, However for the decoupled weight decay paper there is almost no introduction? How much do we introduce without over-burdening the reader in your opinion?}
% The objective of an optimisation algorithm is to 

% \paragraph{Optimisation and Generalisation:}For a data-set of $N$ training input-output samples $\{\vx_i, \vy_i\}$ and a model parametrised by $\vw \in \mathbb{R}^P$, for a given loss function $\ell(h(\vx_{i};\vw),\vy_{i})$ the \emph{empirical risk} also known as the training loss in deep learning is given by $R_{emp}(\vw) = \frac{1}{N}\sum_{i=1}^{N}\ell(h(\vx_{i};\vw),\vy_{i})$. For a randomly sampled mini-batch of size $B$ from the training set, the batch risk is given $R_{batch}(\vw) = \frac{1}{B}\sum_{i=1}^{N}\ell(h(\vx_{i};\vw),\vy_{i})$, which is considered as an estimate of the empirical risk and used in deep learning optimisation. Ideally we would optimise the \emph{true risk}, $R_{true}(\vw) = \int \ell(h(\vx;\vw),\vy_{i})d\phi_{\vx,\vy}$ under the data-generating distribution $\phi_{\vx,\vy}$. The loss using a held out test set can be seen as an unbiased estimate of the true risk.  Given the inherent unobservability of true risk, the minimisation or $R_{emp}$ is considered to be the practical optimisation problem of network training \cite{bottou2018optimization}. The generalisation gap is given by $R_{true}(\vw) - R_{emp}(\vw)$ and can be estimated by reporting the difference between the training and test loss. The adaptive generalisation gap is the difference between the generalisation gaps between adaptive and non adaptive optimisers. Whilst the cross entropy loss $l(h(\vx_{i};\vw),\vy_{i})$ is used in the optimisation procedure, keeping in line with existing literature we will report the frequency of misclassification as a measure of risk. Since for modern DNN's training error is usually very low, we simply report the misclassification on the test set as our measure of generalisation. The nabla $\nabla$ and del $\nabla^{2}$ operators define the gradients and Hessians on the empirical, true and batch risks respectively.
All optimisers minimise the scalar loss $L(\vw_{k})$ for a set of model parameters $\vw_{k} \in \mathbb{R}^P$. The $k+1$-th iteration of a general iterative optimiser at point can be written\footnote{Ignoring additional features such as momentum and explicit regularisations} as:
\begin{equation}
\vw_{k+1} \leftarrow \vw_{k} - \alpha \mB^{-1} \nabla L(\vw_{k}).
\end{equation}
Where $\alpha$ is the global learning rate. For SGD, $\mB = \mI$ whereas for adaptive methods, $\mB$ typically provides some form of approximation to the Hessian $\mB \approx \nabla^{2}L(\vw_{k})$. %(here we omit additional techniques such as momentum and generic regularisers to keep the notation uncluttered since they do not fundamentally change the analysis). %Adaptive gradient methods use past gradient information to create a diagonal approximation to the Hessian.
To take a prominent example, Adam uses the square root of the moving uncentered second moment of the per-parameter gradient \citep{kingma2014adam} which can be interpreted as a running diagonal approximation to the covariance of gradients, which has been argued to be close to the Hessian for DNNs \citep{zhang2019algorithmic,jastrzebski2020the,fort2019stiffness,liu2019variance,he2019local}.
%To analyse the directions of updates produced by a given optimisation algorithm, we employ a quadratic approximation to the local loss surface, $L(\vw_{k})$ at point $\vw_{k} \in \mathbb{R}^P$ and consider the update that would be taken by a second order method. 
Writing this update in the eigenbasis of the Hessian $\mH = \nabla^{2}L(\vw_{k}) = \sum_{i}^{P}\lambda_{i}\vphi_{i}\vphi_{i}^{T} \in \mathbb{R}^{P\times P}$ where $\lambda_1\geq \lambda_2\geq \dots$ represent the ordered scalar eigenvalues, the parameter step takes the form:
\begin{equation}
\label{eq:secondorderopt}
\vw_{k+1} \approx \vw_{k} - \alpha \mH^{-1}\nabla L(\vw_{k}) = \vw_{k} - \sum_{i=1}^{P}\frac{\alpha}{\lambda_{i}+\delta}\vphi_{i}\vphi_{i}^{T}\nabla L(\vw_{k})
\end{equation}
where %$\vw_{k}$ are the model weights at iteration $k$, $[\vphi_{i},\lambda_{i}]$ are the eigenvalues/eigenvector pairs of $\mH$, $\alpha$ is the global learning rate and 
$\delta$ is a damping or numerical stability term. %This damping term, which is typically grid searched \citep{dauphin2014identifying} or adapted during training \citep{martens2015optimizing}, can be interpreted as a trust region that is required to stop the optimiser moving too far in directions deemed flat ($\lambda_{i} \approx 0$) and diverging. 
% Skipping since not really theory
% The exact computation of $\mH^{-1}$ is extremely expensive when $P$ is large (as full eigen-decomposition has computational complexity $\mathcal{O}(P^{3})$) so in practice an approximation is used Hessian-vector products \citep{pearlmutter1994fast} have been used to approximate the Hessian \citep{martens2010deep,dauphin2014identifying}, along with KFAC, which uses a Kronecker factored approximations of the Fisher information matrix \citep{martens2015optimizing}.
The effective learning rate in the flattest ($\lambda \approx 0$) directions  is approximately $\frac{\alpha}{\delta}$, which is larger than that in the sharpest ($\lambda_{i} \gg \delta$) directions  $\frac{\alpha}{\delta+\lambda_{i}}$. Note that the effective learning rate per direction depends of the overlap between the eigen-vector and the gradient $\vphi_{i}^{T}\nabla L(\vw_{k})$, we neglect this for now analyse this in Section \ref{subsec:ia}.
This difference in per direction step size makes the best possible loss reduction under the assumption that the loss function can be effectively modelled by a quadratic. Crucially, however, it does not account for how accurately each eigenvector component of the update estimates the true underlying loss surface. We highlight a particular insight from the spiked covariance literature \citep{johnstone2001distribution} which implies that \textit{sharper directions are estimated more accurately than the flatter directions}.
% REMOVED BECAUSE IT DOESN"T REALLY HELP SUPPORT A CLEAR STORY
% From a dynamical stability perspective \citep{wu2018sgd}, reducing the effective learning rate in the sharp directions means the optimiser is likely to get stuck into a sharp optimum, which generalises worse.
% The key result derived in the spiked covariance literature and recently adapted to the deep learning \citet{granziol2020curvature}, holding under quite general conditions (given in the Appendix), is the following:
This statement is characterised more precisely by the following theorem~\citep{granziol2020curvature}, holding under quite general conditions (given in the Appendix):
\begin{theorem}
	\label{theorem:overlap}
	The eigenvector overlap between the eigenvectors $\hat{\vphi}_{i} \in \mathbb{R}^{P 
		\times 1}$ of the Hessian of the mini-batch $\nabla^{2}L_{batch}(\vw_{k})$ of batch size $B$ and the eigenvectors $\vphi_{i}$ of the Hessian under the expectation of the true data distribution $\nabla^{2}L_{true}(\vw_{k})$, where $L_{true}(\vw_{k}) = \int \ell(\vw_{k};\vx,\vy)d\phi_{\vx,\vy}$ are given by
	\begin{equation}
	|\hat{\vphi}_{i}^{T}\vphi_{i}|^{2} = \begin{cases} 1-\frac{P\sigma^{2}}{B\lambda_{i}^{2}} &\mbox{if } |\lambda_{i}| > \sqrt{\frac{P}{B}}\sigma\\
	0 & \mbox{otherwise} \end{cases}  
	\end{equation}
\end{theorem}
where $\sigma$ captures the sampling noise inherent to representing the data generating distribution with a finite training set. To summarise: the key takeaway of this result is that sharper directions represent possess a better signal-to-noise ratio than flatter directions in estimating the underlying loss surface. In the next section we provide empirical evidence for our conjecture by showing that as we increase the \emph{effective learning rate ratio} in the flat to sharp directions $R_{eff} \equiv \frac{\alpha_{\lambda \approx 0}}{\alpha_{\lambda \gg 0}}$, that generalization decreases. Since the flat directions can be interpreted as being more "noisy" than sharp directions, $R_{eff}$ encapsulates our noise to signal ratio.

% Since the generalization gap is governed by the difference between the empirical and true loss surfaces,  

% Hence the sharp directions represent the signal in our gradient and Equation \ref{eq:secondorderopt} is reduces our signal to noise ratio in our parameter updates. %This is known as the eigenvector phase transition \citep{baik2005phase}. The gradient is a function of curvature\footnote{using a local quadratic expansion $\nabla L = \sum_{i}^{P}\vphi_{i}^{T}\vw(1-\alpha\lambda_{i})\vphi_{i}$} and hence the directions of the true and sampled loss vary is pertinent to generalisation difference. By Theorem \ref{theorem:overlap}, as only the sharpest directions retain information about the true loss, the last thing we want to do is move less in these directions. This is exactly what second order and adaptive gradient methods do, as shown in Equation \ref{eq:adamvssgd}.
% where $\sigma$ captures the sampling noise, present even for the full gradient $B=N$. Hence the sharp directions represent the signal in our gradient and Equation \ref{eq:secondorderopt} is reduces our signal to noise ratio in our parameter updates. %This is known as the eigenvector phase transition \citep{baik2005phase}. The gradient is a function of curvature\footnote{using a local quadratic expansion $\nabla L = \sum_{i}^{P}\vphi_{i}^{T}\vw(1-\alpha\lambda_{i})\vphi_{i}$} and hence the directions of the true and sampled loss vary is pertinent to generalisation difference. By Theorem \ref{theorem:overlap}, as only the sharpest directions retain information about the true loss, the last thing we want to do is move less in these directions. This is exactly what second order and adaptive gradient methods do, as shown in Equation \ref{eq:adamvssgd}.

% \subsection{Implications for Adaptive Gradient Methods} 
% \label{subsec:link}


%The exact computation is extremely expensive when $P$ is large (as full eigen-decomposition has computational complexity $\mathcal{O}(P^{3})$). Hessian vector products \citep{pearlmutter1994fast} have been used to approximate the Hessian \citep{martens2010deep,dauphin2014identifying}, along with KFAC, which uses a Kronecker factored approximations of the Fisher information matrix \citep{martens2015optimizing}. However, more commonly used adaptive gradient methods use past gradient information to create a diagonal approximation to the Hessian. For example, Adam uses the moving uncentered second moment of the per-parameter gradient \cite{kingma2014adam}. 

%. and often grid searched in second order optimisers \citep{dauphin2014identifying}. \citet{chen2018closing} propose the idea that the real generalisation culprit is the small learning rate which typically accompanies adaptive methods.  For flat directions $\lambda \approx 0$, the effective learning rate is $\approx \alpha/\epsilon$, typically much larger for Adam $\approx 10^{4}$ than for for SGD $\approx 10^{-2}$. Since $\alpha$ must be chosen such that $\alpha/\epsilon$ is not too large to prevent divergence, what is much smaller is the effective learning rate for sharp directions of the loss landscape, i.e the directions where $\lambda \gg \epsilon$. Furthermore, as can be seen from Equation \ref{eq:adamvssgd}, effective weight decay in these directions is also very small. 

%Although we do not explicitly calculate curvature information using gradient based methods, the gradient is closely aligned with

% -----------------------------------
% Removing for now up until <<< END
% -----------------------------------
% \begin{figure}[h!]
% 	\centering
% 	\begin{subfigure}[b]{0.45\textwidth}
% 		\includegraphics[width=\textwidth]{figs/IClR_simple_Adam_simple}
% 		\vspace{-15pt}
% 		\caption{Adam various learning rates}
% 		\label{subfig:adaptivegaplr}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{0.49\textwidth}
% 		\includegraphics[width=\textwidth]{figs/IClR_adamvssgd_Adam}
% 		\vspace{-15pt}
% 		\caption{SGD and Adam largest learning rate}
% 		\label{subfig:sgdvsadam}
% 	\end{subfigure}
% 	%	\begin{subfigure}
% 	\vspace{0pt}
% 	\caption{Training and Validation error for Adam/SGD on the VGG-$16$ \& CIFAR-$100$ dataset with no weight decay or batch norm for various learning rates, batch size $B=128$}
% 	\label{fig:lrimportance}
% 	\vspace{-10pt}	
% \end{figure}
% The learning rate to batch size ratio has been shown to correlate with generalisation for SGD \citet{jastrzkebski2017three} and under the dynamical stability perspective of SGD \citet{wu2018sgd}, utilising larger learning rates select flatter minima, which under a Bayesian and minimum description length framework \citet{hochreiter1997flat}, generalise better. For Adam similarly, as shown in Figure \ref{subfig:adaptivegaplr}, larger learning rates lead to better generalisation, despite lower learning rates quickly training better. For this experiment we use the classical VGG-$16$ network \citep{simonyan2014very} and we compare $\alpha = 0.0004$ which is the largest learning rate of stable training\footnote{We test this for multiple seeds.}, to a smaller learning rate. As shown in Figure \ref{subfig:sgdvsadam},
% even when using the respective maximal learning rates for SGD $\alpha=0.01$ and Adam, SGD still generalises better. This is without batch normalisation \citet{ioffe2015batch} or the use of weight decay, so is not addressed in the work of \citet{loshchilov2018decoupled}. Furthermore, even though the global maximal learning rate of Adam is smaller than that of SGD, $\alpha_{Adam} = 0.0004 \ll \alpha_{SGD} = 0.01$, Adam scales its parameter updates by an inverse square root weighted average of gradient squares plus a small offset $\epsilon = 10^{-8}$ for numerical stability. Hence, the largest per parameter learning rate possible is $4\times 10^{4} \gg \alpha_{SGD}$. This shows that whilst effective for SGD, the global learning rate is too crude to analyse the behaviour of adaptive algorithms and a more detailed analysis is required.
% -----------------------------------
% <<< END
% -----------------------------------

\subsection{Empirical Evidence}
\label{subsec:logisticexp}

%To provide evidence in support of our conjecture that relative step sizes taken along the sharpest and flattest directions of the loss play a key role in determining generalization, we conduct two controlled experiments: a small-scale logistic regression task on MNIST and image classification on CIFAR100 with the VGG-16 deep network.

\noindent \textbf{LanczosOPT on Logistic Regression MNIST.} %We validate our conjecture that movements in the sharp direction of the loss landscape are vital to generalisation, as opposed to just stability arguments, we run a convex non stochastic example.
We implement a Lanczos second order (LOPT) \citep{meurant2006lanczos} and gradient descent (GD) optimiser on $1000$ MNIST \citep{lecun1998mnist} training examples with Logistic Regression and validate on a held out test set of $10,000$. The number of well seperated outliers from the spectral bulk is at most the number of classes \citep{papyan2018full} (which is $n_{c}=10$ for this dataset) and we expect that Lanczos algorithm to pick out these well-separated outliers when the number of iterations $k \gg n_{c}$ \citep{granziol2019mlrg,meurant2006lanczos}, so use use $k=50$. To investigate the impact of scaling steps in the Krylov subspace given by the sharpest directions, we consider updates of the form:
\begin{equation}
\label{eq:lanczosopt}
\vw_{k+1} = \vw_{k} -\alpha\bigg(\sum_{i}^{k}\frac{1}{\lambda_{i}+\delta}\vphi_{i}\vphi_{i}^{T}\nabla L(\vw_{k})+\sum_{k+1}^{P}\frac{1}{\delta}\vphi_{i}\vphi_{i}^{T}\nabla L(\vw_{k})\bigg)
\end{equation}
$P=7850$. For fixed $\alpha$, $\delta$ determines the effective learning rate ratio between flat and sharp directions $R_{eff} = \frac{\lambda_{i}}{\delta}+1$. So according to our conjecture if movement in the sharp directions is relevant for generalisation, we should see worse generalisation as we increase $R_{eff}$.
This is exactly what we see in Figure \ref{fig:logisticlrandeps}. Whilst increasing $R_{eff}$ quickly improves training convergence, it damages generalisation. 
%For $\delta = 0.1$ the generalisation performance of LOPT and GD is similar, whereas for all other values it is poorer.

To further evidence for the importance of maintaining movement in the sharpest directions of the loss specifically for generalisation, we introduce two perturbed optimisers (LOPT*/LOPT**), shown as dashed lines of decreasing intensity, where we multiply the eigenvalue in the denominator of Equation \ref{eq:lanczosopt} by $3 \& 10$. This leaves flat directions unperturbed, but further reduces movement in sharp directions. As can be seen from the $\delta = 0.001$ runs in red, whilst all runs achieve a training accuracy of $100\%$, the generalisation difference drops by $1.14\%$, $2.24\%$ respectively. For $\delta = 0.01$, we see an even bigger drop of $4.62\%$ in final test set accuracy with no drop in training for LOPT*, followed by a $4.7\%$ drop in training accuracy and a further drop of $8.55\%$ in testing accuracy for LOPT**. Whilst for larger values of $\delta$ both LOPT*/LOPT** incur reduced training accuracies compared to LOPT, the reduction in generalisation is always far larger.



\begin{figure}[h!]
	\centering
	\vspace{-5pt}
	\begin{subfigure}[b]{0.53\textwidth}
		\includegraphics[width=\textwidth]{figs/Logistic_Gen_train_new}
		%\caption{Training Error}
	\end{subfigure}
	\begin{subfigure}[b]{0.41\textwidth}
		\includegraphics[width=\textwidth]{figs/Logistic_Gen_test_new}
		%\caption{Test Error}
	\end{subfigure}
	%	\begin{subfigure}
	\vspace{-5pt}
	\caption{Training/Test Error for LanczosOPT/GD optimisers on Logistic Regression \& the MNIST dataset with fixed learning rate $\alpha=0.01$ across different damping values, $\delta$.}
	\label{fig:logisticlrandeps}
	\vspace{-15pt}	
\end{figure}
% \subsubsection{}
% \subsection{Experimental Validation: :}
%For the same experimental setup as in Section \ref{sec:motivation}, we plot the training and validation error of the second order optimiser KFAC in Figure \ref{fig:kfaclrandeps}.

\paragraph{KFAC with VGG-16 on CIFAR-100.} To showcase how our conjecture holds for modern deep learning architectures and for the typical settings employed by adaptive optimisers, we run the second order optimiser KFAC \citep{martens2015optimizing} on the VGG-$16$ on the CIFAR-$100$ dataset. By decreasing the global learning rate $\alpha$ whilst keeping the damping to learning rate ratio $\kappa = \frac{\delta}{\alpha}$ constant, we reduce the effective learning rate ratio $R_{eff} = \frac{\lambda_{i}}{\kappa \alpha}+1$.  As shown in Figure \ref{fig:kfaclrandeps}, similar to the Logistic Regression experiment, as we increase $R_{eff}$ the training performance improves slightly $99.85\% \rightarrow 99.92 \%$ and convergence is faster, but the generalisation performance decreases $65\%\rightarrow62.2\%$. 
%The largest learning rate posts a similar generalisation performance to that of SGD $65.3\%$. 

Whilst decreasing the damping results in poor training for large learning rates, for very low learning rates, the network efficiently trains with a lower damping co-efficient. Because such regimes further increase $R_{eff}$, they generalise more poorly. For $\alpha = 0.0001$ dropping the damping co-efficient $\delta$ from to $0.0003$ and $0.0001$ drops the generalisation further to $60.2\%$ and then $56\%$ respectively. Similarly to Logistic Regression, for both cases the drop in generalisation is significantly larger than the drop in training accuracy. We investigate whether the solution generalisation is related to solution sharpness and show the results in Figure \ref{fig:tableofspectralnormkfac}. Lowering the learning rate whilst keeping $\kappa$ constant increase the spectral norm and decreases generalisation. Decreasing $\delta$ whilst keeping $\alpha$ constant, further increases the spectral norm and decreases generalisation. This shows that damping as well as the learning rate is important for flatness and generalisation. 
\begin{figure}[h!]
	\vspace{-20pt}
	\begin{minipage}{0.70\textwidth}
		\begin{subfigure}[b]{0.66\textwidth}
			\includegraphics[width=\textwidth]{figs/gen_train_kfac_VGG16_CIFAR100}
			%		\caption{VGG-16}
		\end{subfigure}
		\hspace{-15pt}
		\begin{subfigure}[b]{0.37\textwidth}
			\includegraphics[width=\textwidth]{figs/gen_test_kfac_VGG16_CIFAR100}
			%		\caption{PRN-110}
		\end{subfigure}
		%	\begin{subfigure}
		\vspace{-20pt}
		\caption{Training/Validation error for KFAC on the VGG-$16$ \& CIFAR-$100$ dataset using various learning rates $\alpha$ and damping $\delta$}
		\label{fig:kfaclrandeps}
		\vspace{-20pt}
	\end{minipage}	
	\begin{minipage}{0.29\textwidth}
		\vspace{25pt}
		\begin{scriptsize}
			\begin{tabular}{@{}llll@{}}
				\toprule
				$\delta \downarrow, \alpha \rightarrow$& 0.01 & 0.001 & 0.0001 \\ \midrule
				0.1 &  \textbf{6.65} & \textbf{} & \textbf{} \\
				0.01 & \textbf{} &  \textbf{20.8} & \textbf{} \\
				0.001 & \textbf{} & \textbf{} & \textbf{48.2} \\
				0.0003 & \textbf{} & \textbf{} &  \textbf{527.2} \\
				0.0001 & \textbf{} & \textbf{} &  \textbf{711.3} \\ \bottomrule
			\end{tabular}
		\end{scriptsize}
		\vspace{6pt}
		\caption{$|\mH|$ at training end for various $\alpha,\delta$}
		\label{fig:tableofspectralnormkfac}
		\vspace{0pt}
	\end{minipage}
\vspace{-20pt}
\end{figure}

%\begin{conjecture}
%	\label{conjecture:main}
%	The step size in the sharpest directions of the loss landscape (as defined by the eigenvectors corresponding to the largest eigenvalues of the Hessian of the loss) is a key explanatory factor of the generalisation performance.
%\end{conjecture}

%We believe that both the generalisation gap between different networks trained with learning rates and the adaptive generalisation gap, can be explained with the following conjecture, which forms the


%To isolate the learning rate from the interfering effects of batch normalisation (BN) \citep{ioffe2015batch} and weight decay (wd) (decoupled or not), we use the classical VGG-$16$ network \citep{simonyan2014very} without batch normalisation and no weight decay on the CIFAR-$100$ dataset classification task. As shown in Figure \ref{subfig:adaptivegaplr}, for Adam similarly to SGD \citep{jastrzkebski2017three}, a large learning rate to batch size ratio leads to greater generalisation. We compare $\alpha = 0.0004$ which is the largest learning rate of stable training\footnote{We test this for multiple seeds.}, to a smaller learning rate.
%We note here that the lower learning rate regime quickly trains better, but generalises worse. Even when using the respective maximal learning rates for SGD and Adam, as shown in Figure \ref{subfig:sgdvsadam}, SGD still generalises better.We believe that both the generalisation gap between different networks trained with learning rates and the adaptive generalisation gap, can be explained with the following conjecture, which forms the focal point of our analysis
%\begin{figure}[h!]
%	\vspace{-10pt}
%	\centering
%	\includegraphics*[width=0.9\textwidth]{figs/IClR_simple_Adam_simple}
%	\vspace{-10pt}
%	\caption{Adam training and validation error curves on the VGG-$16$ network and CIFAR-$100$ dataset, for different learning rates $\alpha$ but fixed batch size $B=128$}
%	\label{fig:adaptivegaplr}
%	\vspace{-10pt}
%\end{figure} 
%which shows the training and test error of the VGG-$16$ without weight decay nor batch normalisation (BN) \citep{ioffe2015batch} for the CIFAR-$100$ dataset under different learning rates. $\alpha = 0.0004$ is the maximal learning rate for which Adam stably trains\footnote{We test this for multiple seeds.} and we compare to another lower learning rate $\alpha = 0.0001$. The experimental details are given in \ref{sec:experimentdetails}. 
%Whilst the mechanisms of how large learning rates aid generalisation are not fully understood, \citet{li2019towards} show that the learning rate size affects the order in which patterns are learned. Specifically that small learning rates are able to memorise small parts of the image which may be spurious \footnote{A well known example of this is the idea that not all sports cars are red, but they often feature in training sets}. 

%\begin{figure}[h!]
%	\vspace{-10pt}
%	\centering
%	\includegraphics*[width=0.9\textwidth]{figs/IClR_adamvssgd_Adam}
%	\vspace{-10pt}
%	\caption{SGD and Adam training/validation error curves on the VGG-$16$ network and CIFAR-$100$ dataset, for different learning rates $\alpha$ but fixed batch size $B=128$}
%	\label{fig:adaptivegap}
%	\vspace{-10pt}
%\end{figure}

\subsection{Prior work increases the step size in sharp directions.} \label{subsec:prior-comp}
Let us consider the update equations for both SGD and Adaptive gradient methods in the basis of the eigenvectors of the Hessian. We assume that the pre-conditioning matrix $\mB \approx \mH$. We also assume that $L2$ regularisation of magnitude $\gamma$ is employed. The $\vw_{k+1}$'th weight vector is then given by:
\begin{equation}
\label{eq:adamvssgd}
\vw_{k+1} = \begin{cases} {\color{blue}{(1-\gamma\alpha)\sum_{i}^{P}\vphi_{i}\vphi_{i}^{T}\vw_{k}}} - {\color{red}{\alpha\sum_{i}^{P}\vphi_{i}^{T}\nabla L(\vw)\vphi_{i}}}\ &\mbox{SGD} \\
{\color{blue}{\sum_{i}^{P}(1-\frac{\gamma\alpha}{\lambda_{i}+\delta})\vphi_{i}\vphi_{i}^{T}\vw_{k}}} - {\color{red}{\alpha\sum_{i}^{P}\frac{\vphi_{i}^{T}\nabla L(\vw)}{\lambda_{i}+\delta}\vphi_{i}}}  & \mbox{Adam} \end{cases}
\end{equation}
% where the damping $\delta$ is set to $10^{-8}$ in Adam.
where the damping $\delta$ is set to $10^{-8}$ in Adam. \emph{Decoupled weight decay} \citet{loshchilov2018decoupled} simply alters Adam such that the {\color{blue}weight decay update term} in Eqn~\ref{eq:adamvssgd} resembles that of SGD instead of that of Adam. This effectively increases the weight decay along the sharpest directions of the loss which in turn increases the effective learning rate in these directions. To demonstrate this point, consider the difference in channel weight vector direction $\hat{\vw_{k}}$ \citep{hoffer2018norm} in the basis of the sharpest eigenvectors after one update of SGD:
\begin{equation}
\label{eq:bndirect}
\sum_{i}^{P}\vphi_{i}\vphi_{i}^{T}\bigg(\hat{\vw}_{k+1}-\hat{\vw}_{k}\bigg) = \frac{-\eta}{||\vw_{k}||^{2}}\bigg(\mI-{\color{purple}{\sum_{i}^{P}\vphi_{i}\hat{\vw_{k}}^{T}\nabla L(\hat{\vw}_{k})\vphi_{i}^{T}\hat{\vw}_{k}}}\bigg)
\end{equation}
Hence decoupled weight decay, which by the {\color{blue} first term} in Equation \ref{eq:adamvssgd} reduces the component along $\vphi_{i}^{T}\hat{\vw_{k}}$, through the reduction of the {\color{purple} corrective term} on the RHS of Eqn. \ref{eq:bndirect}, increases the effective learning rate. 
In Padam \citet{chen2018closing} by changing the square root in the Adam update to an arbitrary power $p < 1/2$, increases both the weight decay and the update in the {\color{red}sharp directions} in Equation \ref{eq:adamvssgd}), increasing the effective learning rate. Epsilon tuning \citep{choi2019empirical}, by increasing both $\epsilon$ and $\alpha$ increases both the {\color{blue}weight decay term} and {\color{red}update in the direction of the sharpest eigenvectors term}.



\subsection{Iterate Averaging: enabling a lower noise to signal ratio}
\label{subsec:ia}

For both Adam and SGD (as shown in Appendix \ref{sec:stepsize}) a larger global learning rate improves generalisation \citet{wu2018sgd,jastrzkebski2017three}. To show how this relates to our conjecture, in the Hessian eigenbasis the SGD updates (Equation \ref{eq:adamvssgd}) have an effective learning rate in the sharp directions is proportional to $\vphi_{i}^{T}\nabla L(\vw_{k})$. The gradient has been shown to have large alignment with the sharpest direction of the loss \citet{gur2018gradient}. Specifically for the CIFAR-$10$ dataset, where we expect there to be at most $10$ well seperated outliers \citep{papyan2018full}. We run the VGG-$16$ network with two learning rates $\alpha \in [0.05,0.01]$ and $L2$ regularisation $\gamma=0.0005$ and show the training/validation curves in Figure \ref{subfig:errcurv} and the gradient overlap as a function of epoch in Figure \ref{subfig:overlap}. We measure the overlap as $\sum_{i=1}^{10}|\vphi_{i}^{T}\nabla L(\vw_{k})|^{2}$

\begin{figure}[h!]
	\centering
	\begin{subfigure}[b]{0.62\textwidth}
		\includegraphics[width=\textwidth]{figs/ICLR_SGD_C10.pdf}
		\vspace{-15pt}
		\caption{SGD various learning rates on CIFAR-$10$}
		\label{subfig:errcurv}
	\end{subfigure}
	\begin{subfigure}[b]{0.35\textwidth}
		\includegraphics[width=\textwidth]{figs/ICLR_SGD_overlap_c10.pdf}
		\vspace{-15pt}
		\caption{Eigenvector Gradient Overlap}
		\label{subfig:overlap}
	\end{subfigure}
	%	\begin{subfigure}
	\vspace{0pt}
	\caption{Train/Val error for the VGG-$16$ \& CIFAR-$10$ dataset with weight decay $\gamma = 0.0005$ and corresponding overlap of the normalised gradient with the sharpest Hessian directions}
	\label{fig:lrsgdimportance}
	\vspace{-10pt}	
\end{figure}

As explained in Section \ref{subsec:framework} and evidenced in Section \ref{subsec:logisticexp} a key driver for the adaptive generalisation gap is the effective learning rate ratio. The damping in Adam is typically fixed at a very small value $\delta = 10^{-8}$ meaning an inherently large effective learning rate ratio. As shown in Figure \ref{subfig:overlap}, large learning rates keep the alignment of the gradient, limiting the effective learning rate ratio. We also note that from Figure \ref{subfig:overlap} that the sharp learning rate decay at the end of training used in typical schedules \footnote{here we use a factor of $100$} massively decreases the overlap with the sharp loss directions. One potential measure to counteract this is to replace the use of covential sharp learning rate decay schedules, with \emph{iterate averaging}.

\textbf{Iterate averaging (IA)} \citep{polyak1992acceleration} performs a simple average of the iterates in the weight space\footnote{an average of the model parameters during training} i.e $\vw_{IA} = 1/n \sum_{i}^{n}\vw_{i}$, where $n$ is the iteration number. IA, along with learning rate reduction, is a key component for traditional convergence proofs \citep{duchi2018introductory}. 
%For the convergence proofs of all gradient based methods the average regret which is bounded can be seen as an upper bound on the loss of the iterate average \cite{duchi2018introductory,duchi2011adaptive,reddi2019convergence} (we elaborate this in App. \ref{sec:optimisationaveraging}). 
IA is optimal for stochastic problems with learning rate decay less than $1/n$, extensively observed in practice \citep{kushner2003stochastic}. As shown in Appendix \ref{subsec:noisyquad}, its noise reduction properties are superior to that exponentially moving averages which is considered to work better in practice \citep{martens2014new,zhang2019lookahead}.
%Despite these strong theoretical results, it has often been labelled as a theoretical tool that is not practically useful possibly due to the worse convergence \cite{trivedi2017}. \citet{defazio2019ineffectiveness} found that when combined with traditional learning rate scheduling IA gave poorer test performance than using the final iterate. 
Recent works have shown that averaging only at the end of training (known as \emph{tail averaging}) whilst maintaining a high learning rate, that generalisation can be significantly improved over that of traditional schedules \citep{izmailov2018averaging,maddox2019simple, merity2017regularizing}. 
The computationally cheaper alternative of averaging every epoch instead of iteration is denoted as \textit{SWA} \citep{izmailov2018averaging}. We compare the importance of averaging frequency in the Appendix \ref{sec:avgfreq}. Despite discussion of its potential in the original Adam paper and its recommendation for transformers \cite{popel2018training}, it is not typically used for image problems. Given that SGD + IA has been shown achieve large scale generalisation performance gains for both image and language problems \citet{merity2017regularizing}, nevertheless it has not achieved widespread adoption with adaptive gradient methods. This begs the question, \textit{why doesn't iterate averaging work well for adaptive optimisers?} and more importantly \textit{can it be made to work well for adaptive optimisers?}

\paragraph{Gadam: Adapting Adam so it works well with Iterate Averaging.}
\label{sec:regularise}
\xingchen{I am now wondering whether we need this section in the main text (I wrote this seciton)... Can we just say Adam+IA doesnt quite work because of the regularisation and relegate the remainder to the appendix?}
Naively combining Adam with IA (AdamIA) does not lead to the same generalisation benefit as SGD with IA (SGD/SWA), as shown in Figure \ref{fig:adamvsadamw}. Model ensembling requires a diverse set of models, i.e a large learning rate. However from Equation \ref{eq:adamvssgd}, movement along the sharpest directions of the loss is much smaller for Adam than for SGD. Hence in these crucial directions, the models are not diverse. One simple remedy for this is to combine IA with decoupled weight decay. As discussed in the previous section, for modern CNNs (which are almost universally equipped with BN), using decoupled weight decay increases the effective learning rate in these directions. we term this amendment to Adam, combining iterate averaging at the tail, decoupled weight decay and large learning rate \textit{Gadam}, which stands for Generalising-Adam to emphasise our focus on test not training performance. We hence expect Gadam to perform better on BN networks.
%Not only does this increase the regularisation effect along these directions, but as modern CNNs are almost universally equipped with normalisation schemes such as BN, weight reduction further acts to maintain an effective learning rate $\alpha_{\mathrm{eff}} \propto \frac{\alpha}{||\vw||^2}$ \cite{zhang2018three}. 
\begin{figure}[h!]
	\vspace{-2mm}
	\centering
	\begin{minipage}{0.6\textwidth}
		\begin{subfigure}[b]{0.49\textwidth}
			\includegraphics[width=\textwidth]{figs/bnvsnobn.png}
			\caption{Validation Accuracy}
		\end{subfigure}
		\begin{subfigure}[b]{0.46\textwidth}
			\includegraphics[width=\textwidth]{figs/ratio.png}
			\caption{Effective LR ${\alpha}/{||\vw||^2}$}
		\end{subfigure}
		\caption{Val. accuracy and $\frac{\alpha}{||\vw||^2}$ of CIFAR-100 \newline on the VGG-$16$ with/without BN. In (b) only results \newline with BN where the quantity is relevant are shown.}
		\label{fig:regularisation}    
	\end{minipage}\hfill
	\begin{minipage}{0.38\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figs/adamlinfnorm.png}  % second figure itself
		\caption{Comparing IA using Adam and AdamW on PRN-110 on CIFAR-100.}
		\label{fig:adamvsadamw}
	\end{minipage}
	\vspace{-10pt}
\end{figure}

To validate our intuition, we run a classical VGG-$16$ network on CIFAR-$100$ with and without BN (Fig. \ref{fig:regularisation}(a)): under the identical set-up, the margin of improvement of Gadam is much larger with BN. While Gadam keeps $\frac{\alpha}{||\vw||^2}$ high, in scheduled AdamW it quickly vanishes once we start learning rate decay, as shown in Figure \ref{fig:regularisation}(b). We consider whether using AdamW without schedules or with more moderate schedules can counteract this effect. However, both alternatives underperform the scheduled AdamW by more than $5\%$ (results not shown in the graph). Revisiting Figure \ref{fig:adamvsadamw} Gadam achieves a generalisation performance on par with SWA while converging faster. The more effective regularisation of AdamW is more directly shown by the much more modest weight norm growth compared to Adam during training (red lines).

%We believe the same regularisation argument also explains why combining adaptive methods with IA has \textit{not} been popularised despite the popularity of the former and the theoretical desiderata of the latter. Indeed we find naively combining Adam with IA is ineffective on typical image problems, but we argue that the real culprit is the ineffective yet commonly used $L_2$ regularisation, which counter-intuitively penalises parameters with more fluctuating gradients \textit{less} than otherwise \cite{loshchilov2018decoupled}, reducing the regularising effect and generalisation benefits IA provides. On the other hand, by penalising parameters equally, AdamW \cite{loshchilov2018decoupled} is a more effective regulariser moderating weight norm increase and we expect IA to be more effective. 

%We validate it Fig. \ref{fig:adamvsadamw}: even though Adam (blue solid lines) performs better than SGD (blue dotted lines) before $T_{\mathrm{avg}}$, the gain from averaging in final accuracy is much less. 




%
%We further argue that IA improves generalisation in networks by maintaining a high \emph{effective} learning rate, which is shown to be a strong regulariser that leads to improved generalisation of Adam and SGD \cite{zhang2018three}. This is obviously made possible by the high (nominal) learning rate schedules of IA, but on networks with batch normalisation (BN), \emph{weight reduction} is also relevant. This can be straightforwardly shown by the Cauchy-Schwartz inequality:
%\begin{theorem}
%	\label{theorem:1}
%	If iterates $\{\vw_i\}$ are drawn from a uniform distribution in the weight space, then the $L_2$ norm of the expected IA point is smaller or equal to the expectation of the $L_2$ weight norm of the iterates: $||\mathbb{E}(\vw_i)||_2^2 \leq \mathbb{E}\big(||\vw_i||_2^2\big)$ (Proof in App. \ref{sec:derivations})
%\end{theorem}
%




 %Given the widespread adoption of adaptive methods, their fast convergence along with the theoretical and practical value of iterate averaging demonstrated on SGD, this question needs further attention and is the subject of this paper.

%Originally optimisation and is actually required in all convergence proofs (we elaborate this in App. \ref{sec:optimisationaveraging}),


%In this work, instead of trading off adaptivity, we propose incorporating  \emph{iterate averaging} (IA) in Adam, an approach we term \textbf{Gadam}, to achieve the same objective. 
%While IA has a strong theoretical foundation in optimisation, it has not been often used in practice until recently:  previous works \cite{izmailov2018averaging, maddox2019simple} have applied IA with first-order optimisers (termed SWA), but to our knowledge the combination of IA and adaptive optimisers has not been thoroughly explored apart from a closely related work \cite{zhang2019lookahead}, which we compare empirically in our paper. Both drawing from prior work and developing new insights in modern deep learning, we first explore theoretically on the mechanisms of action of Gadam and critically examine the oft-held beliefs of IA.  We then empirically show that our algorithm consistently outperforms test performances of finely-tuned SGD and is competitive against SGD with iterate averaging, without compromising adaptivity or introducing sensitive new hyper parameters, in image classification (CIFAR 10/100, ImageNet 32$\times$32) and natural language processing (Penn Treebank, PTB). Finally, we demonstrate the versatility of our approach: we show that by combining Gadam with partial adaptivity (which we term \textbf{GadamX}), empirical results can be further improved, to even outperform SGD with iterate averaging yet still converge faster.

%\subsection{Iterate Averaging}


==> deprecated-drafts/iclr2021_conference.tex <==
%%%% ICLR Macros (LaTex)
%%%% Adapted by Hugo Larochelle from the NIPS stylefile Macros
%%%% Style File
%%%% Dec 12, 1990   Rev Aug 14, 1991; Sept, 1995; April, 1997; April, 1999; October 2014

% This file can be used with Latex2e whether running in main mode, or
% 2.09 compatibility mode.
%
% If using main mode, you need to include the commands
%             \documentclass{article}
%             \usepackage{iclr14submit_e,times}
%

% Change the overall width of the page.  If these parameters are
%       changed, they will require corresponding changes in the
%       maketitle section.
%
\usepackage{eso-pic} % used by \AddToShipoutPicture
\RequirePackage{fancyhdr}
\RequirePackage{natbib}

% modification to natbib citations
\setcitestyle{authoryear,round,citesep={;},aysep={,},yysep={;}}

\renewcommand{\topfraction}{0.95}   % let figure take up nearly whole page
\renewcommand{\textfraction}{0.05}  % let figure take up nearly whole page

% Define iclrfinal, set to true if iclrfinalcopy is defined
\newif\ificlrfinal
\iclrfinalfalse
\def\iclrfinalcopy{\iclrfinaltrue}
\font\iclrtenhv  = phvb at 8pt

% Specify the dimensions of each page

\setlength{\paperheight}{11in}
\setlength{\paperwidth}{8.5in}


\oddsidemargin .5in    %   Note \oddsidemargin = \evensidemargin
\evensidemargin .5in
\marginparwidth 0.07 true in
%\marginparwidth 0.75 true in
%\topmargin 0 true pt           % Nominal distance from top of page to top of
%\topmargin 0.125in
\topmargin -0.625in
\addtolength{\headsep}{0.25in}
\textheight 9.0 true in       % Height of text (including footnotes & figures)
\textwidth 5.5 true in        % Width of text line.
\widowpenalty=10000
\clubpenalty=10000

% \thispagestyle{empty}        \pagestyle{empty}
\flushbottom \sloppy

% We're never going to need a table of contents, so just flush it to
% save space --- suggested by drstrip@sandia-2
\def\addcontentsline#1#2#3{}

% Title stuff, taken from deproc.
\def\maketitle{\par
\begingroup
   \def\thefootnote{\fnsymbol{footnote}}
   \def\@makefnmark{\hbox to 0pt{$^{\@thefnmark}$\hss}} % for perfect author
                                                        % name centering
%   The footnote-mark was overlapping the footnote-text,
%   added the following to fix this problem               (MK)
   \long\def\@makefntext##1{\parindent 1em\noindent
                            \hbox to1.8em{\hss $\m@th ^{\@thefnmark}$}##1}
   \@maketitle \@thanks
\endgroup
\setcounter{footnote}{0}
\let\maketitle\relax \let\@maketitle\relax
\gdef\@thanks{}\gdef\@author{}\gdef\@title{}\let\thanks\relax}

% The toptitlebar has been raised to top-justify the first page

\usepackage{fancyhdr}
\pagestyle{fancy}
\fancyhead{}

% Title (includes both anonimized and non-anonimized versions)
\def\@maketitle{\vbox{\hsize\textwidth
%\linewidth\hsize \vskip 0.1in \toptitlebar \centering
{\LARGE\sc \@title\par}
%\bottomtitlebar % \vskip 0.1in %  minus
\ificlrfinal
    \lhead{Published as a conference paper at ICLR 2021}
    \def\And{\end{tabular}\hfil\linebreak[0]\hfil
            \begin{tabular}[t]{l}\bf\rule{\z@}{24pt}\ignorespaces}%
  \def\AND{\end{tabular}\hfil\linebreak[4]\hfil
            \begin{tabular}[t]{l}\bf\rule{\z@}{24pt}\ignorespaces}%
    \begin{tabular}[t]{l}\bf\rule{\z@}{24pt}\@author\end{tabular}%
\else
       \lhead{Under review as a conference paper at ICLR 2021}
   \def\And{\end{tabular}\hfil\linebreak[0]\hfil
            \begin{tabular}[t]{l}\bf\rule{\z@}{24pt}\ignorespaces}%
  \def\AND{\end{tabular}\hfil\linebreak[4]\hfil
            \begin{tabular}[t]{l}\bf\rule{\z@}{24pt}\ignorespaces}%
    \begin{tabular}[t]{l}\bf\rule{\z@}{24pt}Anonymous authors\\Paper under double-blind review\end{tabular}%
\fi
\vskip 0.3in minus 0.1in}}

\renewenvironment{abstract}{\vskip.075in\centerline{\large\sc
Abstract}\vspace{0.5ex}\begin{quote}}{\par\end{quote}\vskip 1ex}

% sections with less space
\def\section{\@startsection {section}{1}{\z@}{-2.0ex plus
    -0.5ex minus -.2ex}{1.5ex plus 0.3ex
minus0.2ex}{\large\sc\raggedright}}

\def\subsection{\@startsection{subsection}{2}{\z@}{-1.8ex plus
-0.5ex minus -.2ex}{0.8ex plus .2ex}{\normalsize\sc\raggedright}}
\def\subsubsection{\@startsection{subsubsection}{3}{\z@}{-1.5ex
plus      -0.5ex minus -.2ex}{0.5ex plus
.2ex}{\normalsize\sc\raggedright}}
\def\paragraph{\@startsection{paragraph}{4}{\z@}{1.5ex plus
0.5ex minus .2ex}{-1em}{\normalsize\bf}}
\def\subparagraph{\@startsection{subparagraph}{5}{\z@}{1.5ex plus
  0.5ex minus .2ex}{-1em}{\normalsize\sc}}
\def\subsubsubsection{\vskip
5pt{\noindent\normalsize\rm\raggedright}}


% Footnotes
\footnotesep 6.65pt %
\skip\footins 9pt plus 4pt minus 2pt
\def\footnoterule{\kern-3pt \hrule width 12pc \kern 2.6pt }
\setcounter{footnote}{0}

% Lists and paragraphs
\parindent 0pt
\topsep 4pt plus 1pt minus 2pt
\partopsep 1pt plus 0.5pt minus 0.5pt
\itemsep 2pt plus 1pt minus 0.5pt
\parsep 2pt plus 1pt minus 0.5pt
\parskip .5pc


%\leftmargin2em
\leftmargin3pc
\leftmargini\leftmargin \leftmarginii 2em
\leftmarginiii 1.5em \leftmarginiv 1.0em \leftmarginv .5em

%\labelsep \labelsep 5pt

\def\@listi{\leftmargin\leftmargini}
\def\@listii{\leftmargin\leftmarginii
   \labelwidth\leftmarginii\advance\labelwidth-\labelsep
   \topsep 2pt plus 1pt minus 0.5pt
   \parsep 1pt plus 0.5pt minus 0.5pt
   \itemsep \parsep}
\def\@listiii{\leftmargin\leftmarginiii
    \labelwidth\leftmarginiii\advance\labelwidth-\labelsep
    \topsep 1pt plus 0.5pt minus 0.5pt
    \parsep \z@ \partopsep 0.5pt plus 0pt minus 0.5pt
    \itemsep \topsep}
\def\@listiv{\leftmargin\leftmarginiv
     \labelwidth\leftmarginiv\advance\labelwidth-\labelsep}
\def\@listv{\leftmargin\leftmarginv
     \labelwidth\leftmarginv\advance\labelwidth-\labelsep}
\def\@listvi{\leftmargin\leftmarginvi
     \labelwidth\leftmarginvi\advance\labelwidth-\labelsep}

\abovedisplayskip 7pt plus2pt minus5pt%
\belowdisplayskip \abovedisplayskip
\abovedisplayshortskip  0pt plus3pt%
\belowdisplayshortskip  4pt plus3pt minus3pt%

% Less leading in most fonts (due to the narrow columns)
% The choices were between 1-pt and 1.5-pt leading
%\def\@normalsize{\@setsize\normalsize{11pt}\xpt\@xpt} % got rid of @ (MK)
\def\normalsize{\@setsize\normalsize{11pt}\xpt\@xpt}
\def\small{\@setsize\small{10pt}\ixpt\@ixpt}
\def\footnotesize{\@setsize\footnotesize{10pt}\ixpt\@ixpt}
\def\scriptsize{\@setsize\scriptsize{8pt}\viipt\@viipt}
\def\tiny{\@setsize\tiny{7pt}\vipt\@vipt}
\def\large{\@setsize\large{14pt}\xiipt\@xiipt}
\def\Large{\@setsize\Large{16pt}\xivpt\@xivpt}
\def\LARGE{\@setsize\LARGE{20pt}\xviipt\@xviipt}
\def\huge{\@setsize\huge{23pt}\xxpt\@xxpt}
\def\Huge{\@setsize\Huge{28pt}\xxvpt\@xxvpt}

\def\toptitlebar{\hrule height4pt\vskip .25in\vskip-\parskip}

\def\bottomtitlebar{\vskip .29in\vskip-\parskip\hrule height1pt\vskip
.09in} %
%Reduced second vskip to compensate for adding the strut in \@author


%% % Vertical Ruler
%% % This code is, largely, from the CVPR 2010 conference style file
%% % ----- define vruler
%% \makeatletter
%% \newbox\iclrrulerbox
%% \newcount\iclrrulercount
%% \newdimen\iclrruleroffset
%% \newdimen\cv@lineheight
%% \newdimen\cv@boxheight
%% \newbox\cv@tmpbox
%% \newcount\cv@refno
%% \newcount\cv@tot
%% % NUMBER with left flushed zeros  \fillzeros[<WIDTH>]<NUMBER>
%% \newcount\cv@tmpc@ \newcount\cv@tmpc
%% \def\fillzeros[#1]#2{\cv@tmpc@=#2\relax\ifnum\cv@tmpc@<0\cv@tmpc@=-\cv@tmpc@\fi
%% \cv@tmpc=1 %
%% \loop\ifnum\cv@tmpc@<10 \else \divide\cv@tmpc@ by 10 \advance\cv@tmpc by 1 \fi
%%    \ifnum\cv@tmpc@=10\relax\cv@tmpc@=11\relax\fi \ifnum\cv@tmpc@>10 \repeat
%% \ifnum#2<0\advance\cv@tmpc1\relax-\fi
%% \loop\ifnum\cv@tmpc<#1\relax0\advance\cv@tmpc1\relax\fi \ifnum\cv@tmpc<#1 \repeat
%% \cv@tmpc@=#2\relax\ifnum\cv@tmpc@<0\cv@tmpc@=-\cv@tmpc@\fi \relax\the\cv@tmpc@}%
%% % \makevruler[<SCALE>][<INITIAL_COUNT>][<STEP>][<DIGITS>][<HEIGHT>]
%% \def\makevruler[#1][#2][#3][#4][#5]{\begingroup\offinterlineskip
%% \textheight=#5\vbadness=10000\vfuzz=120ex\overfullrule=0pt%
%% \global\setbox\iclrrulerbox=\vbox to \textheight{%
%% {\parskip=0pt\hfuzz=150em\cv@boxheight=\textheight
%% \cv@lineheight=#1\global\iclrrulercount=#2%
%% \cv@tot\cv@boxheight\divide\cv@tot\cv@lineheight\advance\cv@tot2%
%% \cv@refno1\vskip-\cv@lineheight\vskip1ex%
%% \loop\setbox\cv@tmpbox=\hbox to0cm{{\iclrtenhv\hfil\fillzeros[#4]\iclrrulercount}}%
%% \ht\cv@tmpbox\cv@lineheight\dp\cv@tmpbox0pt\box\cv@tmpbox\break
%% \advance\cv@refno1\global\advance\iclrrulercount#3\relax
%% \ifnum\cv@refno<\cv@tot\repeat}}\endgroup}%
%% \makeatother
%% % ----- end of vruler

%% % \makevruler[<SCALE>][<INITIAL_COUNT>][<STEP>][<DIGITS>][<HEIGHT>]
%% \def\iclrruler#1{\makevruler[12pt][#1][1][3][0.993\textheight]\usebox{\iclrrulerbox}}
%% \AddToShipoutPicture{%
%% \ificlrfinal\else
%% \iclrruleroffset=\textheight
%% \advance\iclrruleroffset by -3.7pt
%%   \color[rgb]{.7,.7,.7}
%%   \AtTextUpperLeft{%
%%     \put(\LenToUnit{-35pt},\LenToUnit{-\iclrruleroffset}){%left ruler
%%       \iclrruler{\iclrrulercount}}
%%   }
%% \fi
%% }
%%% To add a vertical bar on the side
%\AddToShipoutPicture{
%\AtTextLowerLeft{
%\hspace*{-1.8cm}
%\colorbox[rgb]{0.7,0.7,0.7}{\small \parbox[b][\textheight]{0.1cm}{}}}
%}


==> deprecated-drafts/intro_deprecated.tex <==
\section{Introduction}\label{sec:intro}
Deep learning's success across a wide variety of tasks, from speech recognition to image classification,
has drawn wide-ranging interest in their optimisation. % algorithms which perform well with deep neural networks.  %, and arguably more important \textit{generalisation}, which aims to improve its ability to infer on the unseen data. 
\textit{Adaptive gradient} optimisers which alter the per parameter learning rate depending on historical gradient information converge significantly faster in training loss than non adaptive methods such as stochastic gradient descent (SGD) with momentum \citep{nesterov2013introductory}. Popular examples include Adam (the most prolific) \citep{kingma2014adam}, AdaDelta \citep{zeiler2012adadelta} and RMSprop \citep{tieleman2012lecture}. However for practical applications, more important than training performance, is the final test set result. The difference between training and test performance is known as the \textit{generalisation gap}. For many image and language problems of interest, the test set performance of adaptive gradient methods is significantly worse than SGD \citep{wilson2017marginal} -- a phenomenon that we term the \textit{adaptive generalisation gap}. As a consequence of this effect, many state-of-the-art models, especially for image classification datasets such as CIFAR \citep{yun2019cutmix} and ImageNet \citep{xie2019selftraining,cubuk2019randaugment} are still trained using SGD with momentum. 
Given the benefits of adaptive methods -- swifter convergence and reduced sensitivity to hyper-parameters relative to SGD -- closing the adaptive generalisation gap has the significant implications, enabling practitioners to attain the performance of finely-tuned SGD schedules at reduced computational cost and environmental impact.

% bringing their test set performance up to or surpassing the level of finely tuned SGD could majorly reduce the cost and environmental impact of deep learning experimentation.
% An understanding of the adaptive generalisation gap is vital for practitioners so they can benefit from the improved convergence of adaptive optimisers. Given that it is already known that adaptive methods are less sensitive to scheduling and hyper-parameter tuning, bringing their test set performance up to or surpassing the level of finely tuned SGD could majorly reduce the cost and environmental impact of deep learning experimentation.
%It is still not well understood \textit{why adaptive methods perform more poorly on the test set.} Much more importantly a holistic understanding of \textit{how we can make adaptive methods post superior test set performance} is still missing. Given the wide spread adoption of both deep learning and adaptive gradient optimisers, we believe that further investigation of both of these questions are of vital theoretical and practical importance to the community.
\paragraph{Related Work} From a theoretical stand point, the learning ratio to batch size ratio has been linked to generalisation \citet{jastrzebski2020the}, which in the case of SGD has been linked to flat minima which generalise better \citep{wu2018sgd}. However to the best of our knowledge there has been no theoretical work analysing the \emph{adaptive generalisation gap}. From a practical perspective, \cite{keskar2017improving} suggest dynamically switching between Adam and SGD; \cite{chen2018closing} devise \textit{Padam}, which introduces a free parameter $p \in [0,1/2]$, where instead of taking the square root of the second moment of the parameter gradient in the preconditioning matrix, now the $p$'th power is taken. This essentially allows the user to toggle between Adam and SGD\footnote{$p=1/2$ reduces to Adam and $p=0$ reduces to SGD with learning rate $\alpha/1+\epsilon$}. The choice of $0 \leq p\leq1/4$ has been shown to have improved convergence properties to that of AMSgrad \citep{zhou2018convergence}. 
\citet{loshchilov2018decoupled} introduce \textit{AdamW}, showing empirically that weight decay instead of $L2$ regularisation improves the generalisation performance of Adam. However as we showcase in Section \ref{sec:experiments}, there has not been a complete success at fully closing the adaptive generalisation gap. Recent work \citet{choi2019empirical} has shown that by \textit{epsilon tuning} (adapting the numerical stability constant\footnote{More specifically, the constant of $\epsilon = 1e^{-8}$ in the denominator of the preconditioning matrix.} used in the implementation of Adam during training), Adam can simulate SGD and retain its generalisation performance. Practically, a setback of applying these methods is that while often improving generalisation, the benefits of adaptivity such as fast convergence are lost. Theoretically, none of these alterations are particularly well motivated. %\citet{loshchilov2018decoupled} link their amendment to Bayesian filtering. 
Neither \citet{keskar2017improving}, \citet{choi2019empirical} nor \cite{chen2018closing} explain why Adam inherently generalises worse than SGD---rather they show that switching from Adam to SGD, or making Adam more like SGD brings improvements. 
%without significant trade-offs (e.g., uniting Adam and SGD often sacrifices fast convergence in return for better generalisation). 
%Furthermore, many of the proposed solutions are heuristically motivated and often lack solid theoretical foundations.
\paragraph{Contributions:} 
In this paper we conjecture that a key driver of the adaptive generalisation gap is the \emph{difference in step sizes taken along the sharpest and flattest directions of the loss landscape}. The fundamental principle underpinning this conjecture---that sharp directions contain information from the underlying process and that flat directions are largely dominated by noise---is theoretically motivated from the spiked covariance model~\citep{baik2004eigenvalues}. 
%This model has been successfully applied in PCA, covariance matrix estimation and finance \citep{bloemendal2016principal, everson2000inferring,bun2017cleaning}. 
Our first key contribution is to show that recent results, derived from the spiked covariance model in the context of deep learning~\citep{granziol2020towards}, provide a principled framework in which to interpret modern developments in improving generalisation of adaptive algorithms, namely \textit{decoupled weight decay} \citep{loshchilov2018decoupled}, \textit{partial adaptivity} \citep{chen2018closing} and \textit{epsilon tuning} \citep{choi2019empirical}. 
Next, motivated by the conjecture above, our second key contribution is to demonstrate that \textit{iterate averaging} in conjunction with larger global learning rates can be employed to increase the effective relative step size along sharper directions of the loss landscape. By integrating this simple technique with existing solvers, 
% As a practical consequence, we posit that by combining the aforementioned techniques with larger global learning rates and iterate averaging, instead of typical sharply decaying learning rate schedules, that the adaptive generalisation gap can be reduced further.
% We introduce this simple amendment as an algorithm 
our final contribution is to introduce \textit{Gadam} (which is fully adaptive like Adam, i.e. $p=1/2$) and its partially adaptive counterpart \textit{GadamX}, where $p=1/8$. 
We demonstrate empirically that Gadam consistently matches or outperforms test performances of finely-tuned SGD, \textit{closing the adaptive generalization gap} for image classification (CIFAR 10/100, ImageNet 32$\times$32, ImageNet) and natural language processing (Penn Treebank, PTB). %We find that for image problems that GadamX further improves empirical results, even outperforming SGD with iterate averaging yet converging faster. 
% We demonstrate empirically that Gadam consistently outperforms test performances of finely-tuned SGD and is competitive against SGD with iterate averaging, without introducing sensitive new hyper parameters, in image classification (CIFAR 10/100, ImageNet 32$\times$32) and natural language processing (Penn Treebank, PTB). We find that for image problems that GadamX further improves empirical results, even outperforming SGD with iterate averaging yet converging faster. 
%Given that one of the goals of adaptive optimisation is to lessen the burden of hyper-parameter tuning, we do not incorporate epsilon tuning \citep{choi2019empirical} into our algorithm, although this could form the basis of interesting future work. In this vein and 
% COULD ADD THIS BACK IN LATER.
% As an interesting further result we show that automated scheduling techniques (which limit the need for tuning) achieve better results for Gadam than they do for SGD with Polyak averaging, which could be of use to practitioners with limited computational budgets.

==> deprecated-drafts/math.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vphi{{\bm{\phi}}}
\def\vepsilon{{\bm{\epsilon}}}
\def\vtheta{{\bm{\theta}}}
\def\vdelta{{\bm{\delta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

